The Selection Problem in Multi-Query Optimization: a Comprehensive Survey

View materialization, index selection, and plan caching are well-known techniques for optimization of query processing in database systems. The essence of these tasks is to select and save a subset of the most useful candidates (views/indexes/plans) for reuse within given space/time budget constraints. In this paper, we propose a unified view on these selection problems. We make a detailed analysis of the root causes of their complexity and summarize techniques to address them. Our survey provides a modern classification of selection algorithms known in the literature, including the latest ones based on Machine Learning. We provide a ground for reuse of the selection techniques between different optimization scenarios and highlight challenges and promising directions in the field. Based on our analysis we derive a method to exponentially accelerate some of the state-of-the-art selection algorithms.

==> problem_modeling.tex <==
\begin{tabular}{ccccc}
    \toprule
    \diagbox{\textbf{parameter}}{\textbf{problem}} & View Selection & Index Selection & Query Caching & Plan Caching \\
    \midrule
    candidate space $\mathcal{C}$   & \multicolumn{3}{c}{data nodes} & subtrees \\
    %\hline
    benefit $\mathcal{B}_c(C)$         & \multicolumn{4}{c}{not a constant in all cases, calculated as the change of the cheapest paths} \\
    %\hline
    limitation $l_c(C)$ & \multicolumn{2}{c}{is not a constant\footnote{under maintenance constraint}} & constant & is not a constant\footnote{when the compressed tree storage technique is used}\\
    \bottomrule
\end{tabular}
